The Last Eight-Billion Years of Intergalactic SiIV Evolution

We identified 24 SiIV absorption systems with z <~ 1 from a blind survey of 49 low-redshift quasars with archival Hubble Space Telescope ultraviolet spectra. We relied solely on the characteristic wavelength separation of the doublet to automatically detect candidates. After visual inspection, we defined a sample of 20 definite (group G = 1) and 4 "highly-likely" (G = 2) doublets with rest equivalent widths W_r for both lines detected at > 3 sigma. The absorber line density of the G = 1 doublets was dN_SiIV/dX = 1.4+0.4/-0.3 for log N(Si+3) > 12.9. The best-fit power law to the G = 1 frequency distribution of column densities f(N(Si+3)) had normalization k = (1.2+0.5/-0.4) x 10^-14 cm2 and slope alpha = -1.6+0.3/-0.3. Using the power-law model of f(N(Si+3)), we measured the Si+3 mass density relative to the critical density: Omega(Si+3) = (3.7+2.8/-1.7) x 10^-8 for 13 < log N(Si+3) < 15. From Monte Carlo sampling of the distributions, we estimated our value to be a factor of 4.8+3.0/-1.9 higher than the 2 < z < 4.5 <Omega(Si+3)>. From a simple linear fit to Omega(Si+3) over the age of the Universe, we estimated a slow and steady increase from z = 5.5 --> 0 with dOmega/dt_age = (0.61+/-0.23) x 10^-8 Gyr^-1. We compared our ionic ratios N(Si+3)/N(C+3) to a 2 < z < 4.5 sample and concluded, from survival analysis, that the two populations are similar, with median <N(Si+3)/N(C+3)> = 0.16.

==> tab2.tex <==
 
 
\begin{deluxetable}{rllllllllll}
\tablewidth{0pc}
\tablecaption{\ion{Si}{4} SYSTEMS SUMMARY \label{tab.sys}}
\tabletypesize{\scriptsize}
\tablehead{ 
\colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)} & 
\colhead{(6)} & \colhead{(7)} & \colhead{(8)} & \colhead{(9)} & \colhead{(10)} & 
\colhead{(11)} \\
\colhead{$z_{1393}$} & \colhead{\dvabs} & 
\colhead{$\lambda_{r}$} & \colhead{\wvlo} & 
\colhead{\wvhi} & \colhead{\EWr} & \colhead{\sigEWr} & 
\colhead{\logN} & \colhead{\siglogN} & 
\colhead{G} & \colhead{Flag} \\ 
 & \colhead{(\!\kms)} & \colhead{(\AA)} & \colhead{(\AA)} & 
\colhead{(\AA)} & \colhead{(\!\mA)} & \colhead{(\!\mA)} & & & & 
}
\startdata
\hline \\[-1ex]
\multicolumn{11}{c}{PG0117+213 ($\zem=1.493$)} \\[1ex]
\hline
0.65536 & \nodata & 1393.76 & 2306.70 & 2307.89 &   273 &    28 & $> 13.73$ & \nodata &  2 & 482 \\
 & $    9.2$ & 1402.77 & 2321.62 & 2322.82 &   122 &    24 & 13.54 &  0.09 &      &   \\
1.04801 & \nodata & 1393.76 & 2853.75 & 2854.89 &   194 &    18 & 13.54 &  0.07 &  1 & 471 \\
 & $  -10.5$ & 1402.77 & 2872.21 & 2873.36 &    83 &    14 & 13.37 &  0.07 &      &   \\
 & $ -111.3$ & 1215.67 & 2486.96 & 2490.84 &  1530 &    21 & $> 14.88$ & \nodata &      &   \\
 & $  -27.2$ & 1206.50 & 2469.68 & 2471.49 &   446 &    19 & $> 13.67$ & \nodata &      &   \\
 & $  -26.2$ & 1260.42 & 2580.19 & 2581.61 &   145 &    11 & 13.16 &  0.03 &      &   \\
\hline \\[-1ex]
\multicolumn{11}{c}{B0312--770 ($\zem=0.223$)} \\[1ex]
\hline
0.20253 & \nodata & 1393.76 & 1674.90 & 1676.82 &   652 &    78 & $> 14.16$ & \nodata &  1 & 511 \\
 & $    7.6$ & 1402.77 & 1685.73 & 1687.67 &   543 &    57 & $> 14.40$ & \nodata &      &   \\
 & $  -15.0$ & 1215.67 & 1460.66 & 1463.09 &  1677 &    20 & $> 14.92$ & \nodata &      &   \\
 & $   -7.3$ & 1025.72 & 1232.52 & 1234.29 &  1139 &    20 & $> 15.59$ & \nodata &      &   \\
 & $   11.2$ &  977.02 & 1174.06 & 1175.78 &   912 &    67 & $> 14.44$ & \nodata &      &   \\
 & $   51.6$ & 1031.93 & 1240.64 & 1241.62 &   496 &    17 & $> 14.94$ & \nodata &      &   \\
 & $   58.2$ & 1037.62 & 1247.48 & 1248.47 &   310 &    14 & 14.87 &  0.02 &      &   \\
 & $   21.7$ & 1206.50 & 1449.82 & 1451.60 &   763 &    19 & $> 13.94$ & \nodata &      &   \\
 & $   61.5$ & 1238.82 & 1489.57 & 1490.45 &   137 &     7 & 13.86 &  0.02 &      &   \\
 & $   62.1$ & 1242.80 & 1494.36 & 1495.24 &    94 &     9 & 13.99 &  0.04 &      &   \\
 & $   39.1$ & 1260.42 & 1515.44 & 1516.45 &   490 &    12 & $> 13.92$ & \nodata &      &   \\
\hline \\[-1ex]
\multicolumn{11}{c}{PKS0405--123 ($\zem=0.573$)} \\[1ex]
\hline
0.16712 & \nodata & 1393.76 & 1626.40 & 1626.95 &   117 &    15 & 13.24 &  0.06 &  1 & 499 \\
 & $    5.4$ & 1402.77 & 1636.92 & 1637.47 &   103 &    23 & 13.49 &  0.10 &      &   \\
 & $  -18.1$ & 1215.67 & 1417.80 & 1419.38 &   876 &    19 & $> 14.60$ & \nodata &      &   \\
 & $   -0.9$ & 1025.72 & 1196.77 & 1197.50 &   444 &    20 & $> 15.19$ & \nodata &      &   \\
 & $  -22.2$ &  977.02 & 1139.53 & 1140.73 &   500 &    22 & $> 14.26$ & \nodata &      &   \\
 & $   12.1$ &  989.80 & 1154.85 & 1155.66 &   214 &    12 & $> 14.64$ & \nodata &      &   \\
 & $  -30.1$ & 1031.93 & 1203.74 & 1204.67 &   391 &    24 & $> 14.77$ & \nodata &      &   \\
 & $  -50.7$ & 1037.62 & 1210.37 & 1211.31 &   218 &    37 & 14.80 &  0.11 &      &   \\
 & $    2.3$ & 1206.50 & 1407.81 & 1408.40 &   236 &    11 & $> 13.38$ & \nodata &      &   \\
 & $   -6.4$ & 1238.82 & 1445.53 & 1446.12 &   108 &    15 & 13.81 &  0.06 &      &   \\
 & $   -7.4$ & 1242.80 & 1450.17 & 1450.76 &    76 &    13 & 13.94 &  0.07 &      &   \\
 & $   -3.3$ & 1260.42 & 1470.73 & 1471.28 &   148 &    12 & $> 13.28$ & \nodata &      &   \\
\hline \\[-1ex]
\multicolumn{11}{c}{PKS0454--22 ($\zem=0.534$)} \\[1ex]
\hline
0.47436 & \nodata & 1393.76 & 2054.25 & 2055.56 &   635 &    52 & $> 13.84$\tablenotemark{a} & \nodata &  1 & 511 \\
 & $   -1.6$ & 1402.77 & 2067.54 & 2068.85 &   475 &    56 & $> 14.02$\tablenotemark{a} & \nodata &      &   \\
 & $  -32.8$ & 1215.67 & 1788.81 & 1795.81 &  3516 &   358 & $> 14.85$ & \nodata &      &   \\
 & $  -20.0$ & 1206.50 & 1778.44 & 1779.02 &   374 &    99 & $> 13.24$\tablenotemark{a} & \nodata &      &   \\
 & $    8.1$ & 1260.42 & 1857.67 & 1859.04 &   617 &    31 & $> 14.03$ & \nodata &      &   \\
 & $    0.0$ & 1548.19 & 2281.82 & 2283.46 &   645 &    37 & $> 14.55$ & \nodata &      &   \\
 & $   -6.2$ & 1550.77 & 2285.62 & 2287.25 &   524 &    33 & $> 14.75$ & \nodata &      &   \\
0.48331 & \nodata & 1393.76 & 2067.11 & 2067.68 &   112 &    37 & $> 13.09$\tablenotemark{a} & \nodata &  1 & 383 \\
 & $    8.4$ & 1402.77 & 2080.48 & 2081.05 & $<   61$ & \nodata & $< 13.34$ & \nodata &      &   \\
 & $   24.2$ & 1215.67 & 1802.80 & 1803.92 &   599 &   105 & $> 14.04$\tablenotemark{a} & \nodata &      &   \\
 & $   -4.4$ & 1206.50 & 1789.01 & 1790.12 &   631 &   124 & $> 13.47$\tablenotemark{a} & \nodata &      &   \\
 & $   -3.8$ & 1260.42 & 1869.08 & 1869.97 &   233 &    21 & $> 13.52$ & \nodata &      &   \\
 & $   -4.2$ & 1548.19 & 2295.80 & 2296.92 &   246 &    27 & 14.04 &  0.08 &      &   \\
 & $   -7.6$ & 1550.77 & 2299.61 & 2300.74 &   183 &    29 & 14.12 &  0.09 &      &   \\
\hline \\[-1ex]
\multicolumn{11}{c}{HE0515--4414 ($\zem=1.710$)} \\[1ex]
\hline
0.68625 & \nodata & 1393.76 & 2349.78 & 2350.71 &   249 &    18 & $< 13.71$\tablenotemark{b} & &  2 & 416 \\
 & $    1.1$ & 1402.77 & 2364.98 & 2365.92 &    68 &    17 & 13.36 &  0.10 &      &   \\
0.94047 & \nodata & 1393.76 & 2703.77 & 2705.23 &   233 &    13 & $< 13.58$\tablenotemark{b} & &  1 & 433 \\
 & $    0.4$ & 1402.77 & 2721.26 & 2722.73 &    56 &    11 & 13.15 &  0.08 &      &   \\
 & $  -15.1$ & 1215.67 & 2357.83 & 2359.83 &   789 &    24 & $> 14.56$ & \nodata &      &   \\
 & $   -1.8$ & 1206.50 & 2340.48 & 2341.68 &   156 &    15 & 13.00 &  0.05 &      &   \\
 & $  -18.4$ & 1260.42 & 2445.04 & 2446.34 &    95 &    17 & 12.90 &  0.08 &      &   \\
 & $   -6.9$ & 1548.19 & 3003.24 & 3005.31 &   365 &    20 & $> 14.27$ & \nodata &      &   \\
 & $   -4.8$ & 1550.77 & 3008.24 & 3010.31 &   242 &    23 & 14.24 &  0.05 &      &   \\
1.14760 & \nodata & 1393.76 & 2992.06 & 2995.16 &   565 &    22 & 13.98 &  0.03 &  1 & 499 \\
 & $    1.0$ & 1402.77 & 3011.41 & 3014.53 &   343 &    29 & 13.98 &  0.04 &      &   \\
 & $  126.9$ & 1215.67 & 2608.01 & 2614.97 &  2976 &    22 & $> 15.18$ & \nodata &      &   \\
 & $  210.9$ & 1206.50 & 2589.59 & 2596.07 &  1961 &    29 & $> 14.31$ & \nodata &      &   \\
 & $   50.5$ & 1238.82 & 2659.38 & 2662.06 &   153 &    18 & 13.91 &  0.05 &      &   \\
 & $   -8.3$ & 1242.80 & 2667.93 & 2670.62 &   259 &    16 & 14.49 &  0.03 &      &   \\
 & $   -3.2$ & 1260.42 & 2705.82 & 2708.53 &   488 &    15 & $> 13.74$ & \nodata &      &   \\
\hline \\[-1ex]
\multicolumn{11}{c}{HS0810+2554 ($\zem=1.510$)} \\[1ex]
\hline
0.55455 & \nodata & 1393.76 & 2166.29 & 2167.04 &   250 &    54 & $> 13.44$\tablenotemark{a} & \nodata &  2 & 354 \\
 & $    4.6$ & 1402.77 & 2180.30 & 2181.05 & $<  160$ & \nodata & $< 14.06$ & \nodata &      &   \\
0.83143 & \nodata & 1393.76 & 2551.82 & 2553.29 &   262 &    30 & 13.67 &  0.08 &  2 & 499 \\
 & $   -0.1$ & 1402.77 & 2568.32 & 2569.80 &   271 &    31 & 13.91 &  0.06 &      &   \\
 & $   49.3$ & 1215.67 & 2225.35 & 2228.26 &  1242 &   106 & $> 14.61$ & \nodata &      &   \\
 & $   23.5$ & 1206.50 & 2209.27 & 2210.36 &   380 &    62 & $> 13.25$\tablenotemark{a} & \nodata &      &   \\
 & $  -13.1$ & 1548.19 & 2834.27 & 2836.40 &   774 &    49 & $> 14.63$ & \nodata &      &   \\
 & $  -10.3$ & 1550.77 & 2838.99 & 2841.12 &   724 &    53 & $> 14.89$ & \nodata &      &   \\
\hline \\[-1ex]
\multicolumn{11}{c}{MARK132 ($\zem=1.757$)} \\[1ex]
\hline
0.93166 & \nodata & 1393.76 & 2691.35 & 2692.92 &    73 &    12 & 12.95 &  0.07 &  2 & 467 \\
 & $  -19.2$ & 1402.77 & 2708.76 & 2710.34 &    86 &    12 & $< 13.31$\tablenotemark{b} & &      &   \\
\hline \\[-1ex]
\multicolumn{11}{c}{PG1116+215 ($\zem=0.176$)} \\[1ex]
\hline
0.13846 & \nodata & 1393.76 & 1586.58 & 1586.87 &    34 &     9 & 12.68 &  0.10 &  1 & 383 \\
 & $   -5.0$ & 1402.77 & 1596.84 & 1597.13 & $<   18$ & \nodata & $< 12.64$ & \nodata &      &   \\
 & $    9.9$ & 1215.67 & 1383.52 & 1384.48 &   475 &     6 & $> 14.37$ & \nodata &      &   \\
 & $    5.0$ & 1025.72 & 1167.48 & 1168.07 &   317 &    18 & $> 15.01$ & \nodata &      &   \\
 & $    9.2$ &  977.02 & 1112.23 & 1112.67 &   114 &     7 & $> 13.60$ & \nodata &      &   \\
 & $   13.5$ &  989.80 & 1126.59 & 1127.21 &    73 &     8 & 14.06 &  0.04 &      &   \\
 & $    0.6$ & 1031.93 & 1174.49 & 1175.13 &    69 &    12 & 13.86 &  0.07 &      &   \\
 & $    3.5$ & 1037.62 & 1180.97 & 1181.61 &    48 &    13 & 13.97 &  0.11 &      &   \\
 & $    4.4$ & 1206.50 & 1373.41 & 1373.75 &    85 &     5 & $> 12.91$ & \nodata &      &   \\
 & $    1.6$ & 1260.42 & 1434.78 & 1435.13 &    52 &     3 & 12.74 &  0.02 &      &   \\
\hline \\[-1ex]
\multicolumn{11}{c}{PG1206+459 ($\zem=1.155$)} \\[1ex]
\hline
0.92690 & \nodata & 1393.76 & 2682.15 & 2687.93 &   777 &    19 & 14.08 &  0.01 &  1 & 477 \\
 & $   33.2$ & 1402.77 & 2699.50 & 2705.31 &   402 &    29 & 14.06 &  0.03 &      &   \\
 & $  -35.5$ & 1215.67 & 2339.49 & 2345.04 &  2384 &    30 & $> 15.07$ & \nodata &      &   \\
 & $   50.6$ & 1206.50 & 2321.95 & 2326.84 &   968 &    39 & $> 13.97$ & \nodata &      &   \\
 & $ -113.6$ & 1238.82 & 2384.39 & 2388.91 &   870 &    38 & $> 14.85$ & \nodata &      &   \\
 & $ -118.5$ & 1242.80 & 2392.06 & 2396.59 &   498 &    33 & 14.82 &  0.03 &      &   \\
 & $   81.1$ & 1260.42 & 2427.35 & 2430.55 &   429 &    24 & $> 13.73$ & \nodata &      &   \\
 & $  -33.6$ & 1548.19 & 2979.54 & 2985.63 &  2265 &    59 & $> 15.13$ & \nodata &      &   \\
 & $  -96.8$ & 1550.77 & 2984.50 & 2990.59 &  2151 &    54 & $> 15.38$ & \nodata &      &   \\
0.93429 & \nodata & 1393.76 & 2695.43 & 2696.40 &   143 &    11 & $> 13.51$ & \nodata &  1 & 511 \\
 & $   -2.3$ & 1402.77 & 2712.87 & 2713.84 &    98 &    11 & 13.60 &  0.06 &      &   \\
 & $  -20.3$ & 1215.67 & 2350.48 & 2352.09 &   552 &    21 & $> 14.42$ & \nodata &      &   \\
 & $   -3.3$ & 1206.50 & 2333.27 & 2334.11 &   133 &    15 & $> 13.13$ & \nodata &      &   \\
 & $   -5.9$ & 1548.19 & 2993.93 & 2995.25 &   259 &    22 & $> 14.18$ & \nodata &      &   \\
 & $   -5.4$ & 1550.77 & 2998.91 & 3000.23 &   200 &    20 & $> 14.34$ & \nodata &      &   \\
\hline \\[-1ex]
\multicolumn{11}{c}{PG1211+143 ($\zem=0.081$)} \\[1ex]
\hline
0.05118 & \nodata & 1393.76 & 1464.88 & 1465.29 &    66 &     4 & 12.96 &  0.03 &  1 & 509 \\
 & $    0.4$ & 1402.77 & 1474.35 & 1474.76 &    44 &     5 & 13.04 &  0.05 &      &   \\
 & $   24.1$ & 1215.67 & 1277.06 & 1279.19 &  1213 &     7 & $> 14.74$ & \nodata &      &   \\
 & $   13.9$ & 1025.72 & 1077.52 & 1079.46 &   846 &    19 & $> 15.39$ & \nodata &      &   \\
 & $  -62.0$ &  977.02 & 1026.58 & 1027.04 &   304 &    85 & $> 13.67$\tablenotemark{a} & \nodata &      &   \\
 & $    0.1$ & 1206.50 & 1267.90 & 1268.38 &   135 &     4 & 12.97 &  0.01 &      &   \\
 & $    9.2$ & 1260.42 & 1324.83 & 1325.13 &    27 &     3 & 12.35 &  0.04 &      &   \\
 & $  -12.0$ & 1548.19 & 1626.83 & 1627.67 &   264 &    10 & $> 14.07$ & \nodata &      &   \\
 & $   -8.2$ & 1550.77 & 1629.54 & 1630.38 &   147 &    10 & 14.01 &  0.03 &      &   \\
\hline \\[-1ex]
\multicolumn{11}{c}{MRK205 ($\zem=0.071$)} \\[1ex]
\hline
0.00428 & \nodata & 1393.76 & 1399.43 & 1400.00 &   122 &    11 & 13.25 &  0.04 &  1 & 511 \\
 & $   -2.4$ & 1402.77 & 1408.48 & 1409.05 &    75 &    13 & 13.33 &  0.07 &      &   \\
 & $    7.6$ & 1215.67 & 1220.38 & 1221.47 &   807 &    32 & $> 14.53$ & \nodata &      &   \\
 & $    9.6$ & 1025.72 & 1029.68 & 1030.64 &   486 &    29 & $> 15.23$ & \nodata &      &   \\
 & $  -10.4$ &  977.02 &  980.81 &  981.56 &   382 &    46 & $> 14.13$ & \nodata &      &   \\
 & $    0.9$ &  989.80 &  993.68 &  994.38 &   301 &    41 & $> 14.51$\tablenotemark{a} & \nodata &      &   \\
 & $    4.7$ & 1206.50 & 1211.42 & 1211.97 &   263 &    32 & $> 13.09$\tablenotemark{a} & \nodata &      &   \\
 & $    4.6$ & 1260.42 & 1265.57 & 1266.25 &   240 &    11 & $> 13.54$ & \nodata &      &   \\
 & $   -3.7$ & 1548.19 & 1554.46 & 1555.20 &   292 &    23 & $> 14.14$ & \nodata &      &   \\
 & $    4.9$ & 1550.77 & 1557.05 & 1557.78 &   196 &    23 & $> 14.17$ & \nodata &      &   \\
\hline \\[-1ex]
\multicolumn{11}{c}{QSO--123050+011522 ($\zem=0.117$)} \\[1ex]
\hline
0.00572 & \nodata & 1393.76 & 1401.47 & 1401.92 &    66 &     8 & 12.96 &  0.05 &  1 & 511 \\
 & $   -3.0$ & 1402.77 & 1410.54 & 1410.99 &    63 &     9 & 13.21 &  0.06 &      &   \\
 & $  -13.1$ & 1215.67 & 1222.14 & 1222.95 &   597 &    16 & $> 14.45$ & \nodata &      &   \\
 & $   -4.9$ & 1206.50 & 1213.19 & 1213.59 &   175 &    34 & $> 12.91$\tablenotemark{a} & \nodata &      &   \\
 & $   -7.7$ & 1260.42 & 1267.41 & 1267.77 &    74 &    11 & 12.83 &  0.07 &      &   \\
 & $    6.9$ & 1548.19 & 1556.92 & 1557.30 &    67 &    12 & 13.35 &  0.08 &      &   \\
 & $   12.6$ & 1550.77 & 1559.51 & 1559.89 &    46 &    12 & 13.44 &  0.11 &      &   \\
\hline \\[-1ex]
\multicolumn{11}{c}{PG1248+401 ($\zem=1.032$)} \\[1ex]
\hline
0.77305 & \nodata & 1393.76 & 2470.19 & 2473.26 &   472 &    19 & $> 14.01$ & \nodata &  1 & 495 \\
 & $    4.1$ & 1402.77 & 2486.17 & 2489.26 &   348 &    17 & 14.06 &  0.02 &      &   \\
 & $  -23.5$ & 1548.19 & 2743.66 & 2745.76 &   625 &    36 & $> 14.56$ & \nodata &      &   \\
 & $  -19.8$ & 1550.77 & 2748.22 & 2750.33 &   569 &    31 & $> 14.77$ & \nodata &      &   \\
0.85485 & \nodata & 1393.76 & 2584.38 & 2585.90 &   211 &    21 & 13.49 &  0.05 &  1 & 495 \\
 & $   -9.8$ & 1402.77 & 2601.10 & 2602.63 &   138 &    31 & 13.59 &  0.10 &      &   \\
 & $  -37.6$ & 1260.42 & 2337.12 & 2338.52 &   197 &    27 & 13.34 &  0.11 &      &   \\
 & $   38.4$ & 1548.19 & 2870.57 & 2873.99 &   826 &    39 & $> 14.59$ & \nodata &      &   \\
 & $   26.9$ & 1550.77 & 2875.34 & 2878.77 &   567 &    41 & $> 14.65$ & \nodata &      &   \\
\hline \\[-1ex]
\multicolumn{11}{c}{PG1630+377 ($\zem=1.476$)} \\[1ex]
\hline
0.91432 & \nodata & 1393.76 & 2667.64 & 2668.60 &   123 &    15 & 13.26 &  0.06 &  1 & 497 \\
 & $    0.1$ & 1402.77 & 2684.89 & 2685.86 &    98 &    12 & 13.47 &  0.06 &      &   \\
 & $   10.6$ & 1215.67 & 2325.82 & 2328.60 &  1076 &    33 & $> 14.69$ & \nodata &      &   \\
 & $   21.0$ & 1206.50 & 2309.25 & 2310.48 &   145 &    19 & 13.00 &  0.07 &      &   \\
 & $    9.5$ & 1548.19 & 2963.25 & 2965.06 &   413 &    16 & $> 14.31$ & \nodata &      &   \\
 & $   22.9$ & 1550.77 & 2968.18 & 2969.99 &   317 &    18 & $> 14.43$ & \nodata &      &   \\
0.95279 & \nodata & 1393.76 & 2720.92 & 2722.40 &   202 &    15 & 13.49 &  0.04 &  1 & 499 \\
 & $    8.4$ & 1402.77 & 2738.52 & 2740.01 &   136 &    21 & 13.59 &  0.07 &      &   \\
 & $   53.5$ & 1215.67 & 2372.75 & 2375.93 &  1400 &    23 & $> 14.83$ & \nodata &      &   \\
 & $   -5.8$ & 1206.50 & 2355.41 & 2356.56 &   157 &    19 & 13.00 &  0.06 &      &   \\
 & $  -10.9$ & 1260.42 & 2460.75 & 2461.75 &    45 &    13 & 12.56 &  0.12 &      &   \\
 & $  -14.7$ & 1548.19 & 3022.00 & 3023.80 &   560 &    21 & $> 14.43$ & \nodata &      &   \\
 & $  -39.0$ & 1550.77 & 3027.02 & 3028.83 &   280 &    22 & 14.27 &  0.04 &      &   \\
\hline \\[-1ex]
\multicolumn{11}{c}{PG1634+706 ($\zem=1.334$)} \\[1ex]
\hline
0.65351 & \nodata & 1393.76 & 2303.95 & 2305.30 &   145 &    11 & 13.30 &  0.04 &  1 & 499 \\
 & $   -2.4$ & 1402.77 & 2318.85 & 2320.21 &    71 &     9 & 13.25 &  0.06 &      &   \\
 & $    8.2$ & 1215.67 & 2009.41 & 2010.92 &   630 &    30 & $> 14.45$ & \nodata &      &   \\
 & $  -23.2$ & 1206.50 & 1994.50 & 1995.48 &   297 &    22 & $> 13.46$ & \nodata &      &   \\
 & $    8.8$ & 1548.19 & 2559.26 & 2560.56 &   385 &    10 & $> 14.29$ & \nodata &      &   \\
 & $    6.8$ & 1550.77 & 2563.51 & 2564.81 &   271 &    10 & 14.31 &  0.02 &      &   \\
0.81813 & \nodata & 1393.76 & 2533.54 & 2534.40 & $<   15$ & \nodata & $< 12.25$ & \nodata &  2 & 243 \\
 & $   -2.5$ & 1402.77 & 2549.93 & 2550.79 &    21 &     7 & 12.71 &  0.13 &      &   \\
 & $    0.8$ & 1215.67 & 2209.74 & 2210.75 &   201 &    10 & $> 13.92$ & \nodata &      &   \\
 & $    2.2$ & 1206.50 & 2193.47 & 2193.91 &    41 &     6 & 12.38 &  0.07 &      &   \\
 & $   -1.4$ & 1260.42 & 2291.25 & 2291.88 &    21 &     6 & 12.21 &  0.13 &      &   \\
 & $    0.6$ & 1548.19 & 2814.31 & 2815.37 &    90 &     5 & 13.51 &  0.02 &      &   \\
 & $    1.1$ & 1550.77 & 2818.99 & 2820.05 &    69 &     5 & 13.63 &  0.03 &      &   \\
0.90560 & \nodata & 1393.76 & 2655.66 & 2656.10 &   182 &     4 & $< 13.68$\tablenotemark{b} & &  1 & 433 \\
 & $   -4.7$ & 1402.77 & 2672.83 & 2673.28 &    32 &     5 & 12.92 &  0.07 &      &   \\
 & $    0.5$ & 1215.67 & 2315.94 & 2317.38 &   329 &     8 & $> 14.17$ & \nodata &      &   \\
 & $   -4.7$ & 1025.72 & 1954.17 & 1955.03 &   182 &    21 & $> 14.39$\tablenotemark{a} & \nodata &      &   \\
 & $   -3.5$ & 1031.93 & 1966.01 & 1966.81 &   104 &    22 & 14.08 &  0.10 &      &   \\
 & $   -6.3$ & 1037.62 & 1976.85 & 1977.66 &    67 &    18 & 14.11 &  0.12 &      &   \\
 & $    1.2$ & 1206.50 & 2298.70 & 2299.53 &    61 &     8 & 12.58 &  0.05 &      &   \\
 & $    2.2$ & 1238.82 & 2360.45 & 2361.00 &    67 &     6 & 13.57 &  0.04 &      &   \\
 & $   -8.0$ & 1242.80 & 2368.04 & 2368.59 &    52 &     5 & 13.74 &  0.05 &      &   \\
 & $  -12.5$ & 1260.42 & 2401.61 & 2402.39 &    89 &     5 & 12.94 &  0.03 &      &   \\
 & $    1.1$ & 1548.19 & 2949.56 & 2950.92 &   198 &     8 & 14.04 &  0.04 &      &   \\
 & $    0.1$ & 1550.77 & 2954.46 & 2955.82 &   167 &     8 & 14.21 &  0.03 &      &   \\
0.99035 & \nodata & 1393.76 & 2773.22 & 2774.74 &   240 &     7 & 13.73 &  0.02 &  1 & 503 \\
 & $   -1.3$ & 1402.77 & 2791.16 & 2792.69 &   162 &     6 & 13.74 &  0.02 &      &   \\
 & $  -13.1$ & 1215.67 & 2417.15 & 2421.89 &  1142 &    11 & $> 14.73$ & \nodata &      &   \\
 & $   -0.1$ & 1025.72 & 2040.59 & 2042.46 &   650 &    21 & $> 15.34$ & \nodata &      &   \\
 & $   -3.1$ &  977.02 & 1944.01 & 1945.25 &   342 &    22 & $> 14.08$ & \nodata &      &   \\
 & $    2.4$ &  989.80 & 1969.74 & 1970.38 &    84 &    20 & 14.13 &  0.12 &      &   \\
 & $   -7.5$ & 1031.93 & 2053.55 & 2054.09 &   126 &    12 & 14.13 &  0.06 &      &   \\
 & $  -10.0$ & 1037.62 & 2064.87 & 2065.42 &    44 &    12 & 13.92 &  0.13 &      &   \\
 & $   -3.6$ & 1206.50 & 2400.57 & 2402.41 &   396 &     6 & $> 13.66$ & \nodata &      &   \\
 & $  -21.5$ & 1260.42 & 2507.89 & 2509.16 &   254 &     7 & $> 13.63$ & \nodata &      &   \\
1.04106 & \nodata & 1393.76 & 2842.77 & 2845.68 &   167 &     5 & 13.32 &  0.02 &  1 & 477 \\
 & $  -11.0$ & 1402.77 & 2861.15 & 2864.09 &    96 &     8 & 13.35 &  0.03 &      &   \\
 & $  -34.7$ & 1215.67 & 2479.06 & 2483.03 &  1433 &    11 & $> 14.87$ & \nodata &      &   \\
 & $  -28.9$ & 1025.72 & 2091.78 & 2094.72 &  1090 &    24 & $> 15.58$ & \nodata &      &   \\
 & $  -34.5$ &  977.02 & 1992.55 & 1995.15 &   780 &    30 & $> 14.42$ & \nodata &      &   \\
 & $  -62.8$ & 1031.93 & 2104.64 & 2107.27 &   348 &    20 & 14.61 &  0.03 &      &   \\
 & $  -42.3$ & 1037.62 & 2116.25 & 2118.89 &   297 &    21 & 14.79 &  0.03 &      &   \\
 & $    7.2$ & 1206.50 & 2461.01 & 2463.35 &   422 &     9 & 13.54 &  0.02 &      &   \\
 & $   44.1$ & 1260.42 & 2572.37 & 2573.51 &    44 &     7 & 12.53 &  0.07 &      &   \\
\hline \\[-1ex]
\multicolumn{11}{c}{PHL1811 ($\zem=0.190$)} \\[1ex]
\hline
0.08094 & \nodata & 1393.76 & 1506.37 & 1506.76 &   108 &     7 & $> 13.44$ & \nodata &  1 & 509 \\
 & $    0.2$ & 1402.77 & 1516.12 & 1516.51 &    74 &     9 & 13.45 &  0.05 &      &   \\
 & $  -36.1$ & 1215.67 & 1313.15 & 1314.77 &   904 &     9 & $> 14.64$ & \nodata &      &   \\
 & $  -55.0$ & 1025.72 & 1108.07 & 1109.17 &   703 &    11 & $> 15.40$ & \nodata &      &   \\
 & $  -29.8$ &  977.02 & 1055.44 & 1056.24 &   335 &    10 & $> 14.07$ & \nodata &      &   \\
 & $   -1.9$ &  989.80 & 1069.57 & 1070.02 &   138 &     9 & $> 14.47$ & \nodata &      &   \\
 & $    2.8$ & 1206.50 & 1304.00 & 1304.26 &   177 &     4 & $> 13.31$ & \nodata &      &   \\
 & $   -6.0$ & 1260.42 & 1362.30 & 1362.65 &   172 &     4 & $> 13.44$ & \nodata &      &   \\
 & $   -8.3$ & 1548.19 & 1672.94 & 1673.74 &   179 &    27 & $> 13.92$\tablenotemark{a} & \nodata &      &   \\
 & $  -11.4$ & 1550.77 & 1675.72 & 1676.53 &   131 &    23 & 14.03 &  0.10 &      &   \\
\enddata
\tablenotetext{a}{COG.}
\tablenotetext{b}{Blended.}
\tablecomments{Si\,IV systems by target and redshift of Si\,IV 1393.
Upper limits are $2\sigma$ limits for both \EWr\ and \logN.
The column densities were measured by the AODM, unless ``COG'' is indicated, in which case, the limit is from assuming \EWr\ results from the linear portion of the COG.
The definite Si\,IV doublets are labeled group G = 1, while the ``highly-likely'' doublets are G = 2.
The binary flag is described in Section \ref{sec.selec}.
}
\end{deluxetable}

